Bridging theory and observations in stellar pulsations: The impact of convection and metallicity on the instability strips of Classical and Type-II Cepheids

The effect of metallicity on the theoretical and empirical period-luminosity (PL) relations of Cepheid variables is not well understood and remains a highly debated issue. Here, we examine empirical colour-magnitude diagrams (CMDs) of Classical and Type-II Cepheids in the Magellanic Clouds and compare those with the theoretically predicted instability strip (IS) edges. We explore the effects of incorporating turbulent flux, turbulent pressure, and radiative cooling into the convection theory on the predicted IS at various metallicities using MESA-RSP. We find that the edges become redder with the increasing complexity of convection physics incorporated in the fiducial convection sets, and are similarly shifted to the red with increasing metallicity. The inclusion of turbulent flux and pressure improves the agreement of the red edge of the IS, while their exclusion leads to better agreement with observations of the blue edge. About 90% of observed stars are found to fall within the predicted bluest and reddest edges across the considered variations of turbulent convection parameters. Furthermore, we identify and discuss discrepancies between theoretical and observed CMDs in the low effective temperature and high luminosity regions for stars with periods greater than ~ 20 days. These findings highlight the potential for calibrating the turbulent convection parameters in stellar pulsation models or the prediction of a new class of rare, long-period, 'red Cepheids', thereby improving our understanding of Cepheids and their role in cosmological studies.

==> quant_temp.tex <==


\begin{table*}
        \centering
        \caption{$T_{\rm eff}$ for FU CCs, FO CCs and T2Cs obtained from Gaussian fitting using different metallicities and different sets of turbulent convection parameters.}
        \label{table:quant_temp}
        \begin{tabular}{|c|c|c|c|c|c|c|} % four columns, alignment for each
        \hline
		Class of Variable & Metal Fraction ($Z$) & \multicolumn{4}{c|}{Mean $T_{\rm eff}$ [K]}  \\ \cline{3-6}
			   &                 & Set A & Set B & Set C & Set D \\ \hline
		FU CCs            &All             &$5731$&$5734$&$5484$&$5514$\\
			              &$0.013$		 &$5644$&$5639$&$5327$&$5365$ \\
			              &$0.00609$              &$5741$&$5750$&$5510$&$5541$ \\
			              &$0.0024$              &$5793$&$5806$&$5592$&$5624$ \\ \hline
        FO CCs            &All              &$6356$&$6240$&$6165$&$6049$\\
			              &$0.013$		 &$6375$&$6220$&$6185$&$6007$ \\
			              &$0.00609$              &$6334$&$6240$&$6136$&$6056$ \\
			              &$0.0024$              &$6316$&$6241$&$6123$&$6070$ \\ \hline
        T2Cs            &All              &$5701$&$5726$&$5532$&$5590$ \\
			              &$0.013$		    &$5593$&$5583$&$5391$&$5454$ \\
                        &$0.00834$		 &$5633$&$5641$&$5456$&$5513$ \\
                        &$0.00424$		 &$5672$&$5706$&$5492$&$5551$ \\
                        &$0.00135$		 &$5731$&$5752$&$5561$&$5622$ \\
			              &$0.00061$        &$5738$&$5754$&$5583$&$5633$ \\
			              &$0.00043$        &$5741$&$5767$&$5584$&$5637$ \\ 
                        &$0.00014$		 &$5749$&$5768$&$5583$&$5633$ \\\hline

	
        \end{tabular}
\end{table*}



==> star_nc.tex <==
\begin{table*}
        \centering
        \caption{Number of  observed stars within the estimated IS edges for FU CCs, FO CCs and T2Cs.}
        \label{table:star_counts}
        \begin{tabular}{|c|c|c|c|c|c|c|} % four columns, alignment for each
        \hline
		\multirow{4}{*}{Class of Variables} &\multicolumn{2}{c|}{FU CCs} & \multicolumn{2}{c|}{FO CCs} & \multicolumn{2}{c|}{T2Cs} \\  \cline{2-7} 
                                          & LMC ($\%$) & SMC ($\%$) & LMC ($\%$) & SMC ($\%$) &LMC ($\%$)&SMC ($\%$) \\ \hline
                A              &$96.86$&$93.14$&$92.28$&$92.41$&$93.54$&$90.91$ \\ 
			   B		     &$96.71$&$94.76$&$95.18$&$96.28$&$92.90$&$90.91$ \\
    			   C              &$97.56$&$97.14$&$68.29$&$69.56$&$85.81$&$84.84$ \\
    			   D              &$98.18$&$97.32$&$89.92$&$88.68$&$85.81$&$84.84$ \\ 
                ALL sets &$99.94$ & $99.48$ & $96.18$&$97.08$&$94.83$& $90.91$ \\ \hline
        \end{tabular}
\end{table*}

